TERA: the Toxicological Effect and Risk Assessment Knowledge Graph

Ecological risk assessment requires large amounts of chemical effect data from laboratory experiments. Due to experimental effort and animal welfare concerns it is desired to extrapolate data from existing sources. To cover the required chemical effect data several data sources need to be integrated to enable their interoperability. In this paper we introduce the Toxicological Effect and Risk Assessment (TERA) knowledge graph, which aims at providing such integrated view, and the data preparation and steps followed to construct this knowledge graph. We also present the applications of TERA for chemical effect prediction and the potential applications within the Semantic Web community.

==> effect_example.tex <==
\begin{tikzcd}
\texttt{ecotox:LC50}    &  & \texttt{ecotox:Result}                                                                                                                                                                                                                                                        &  & \texttt{ncbi:taxon/555} \\
                        &  & \texttt{\_:b2} \arrow[u, "\texttt{rdf:type}" description] \arrow[rru, "\texttt{ecotox:species}" description] \arrow[lld, "\texttt{ecotox:compound}" description] \arrow[rrd, "\texttt{ecotox:concentration}" description] \arrow[llu, "\texttt{ecotox:endpoint}" description] &  &                         \\
\texttt{obo:CHEBI\_7071} &  &                                                                                                                                                                                                                                                                               &  & 0.5                    
\end{tikzcd}

==> sibling_example.tex <==
\begin{tikzcd}
                                                                           & \texttt{ncbi:Taxon}                                                                                                   &  &                         \\
                                                                           & \texttt{\_:b1} \arrow[rrd, "\texttt{$\hat{~}$rdfs:subClassOf}" description] \arrow[u, "\texttt{rdf:type}" description] &  &                         \\
\texttt{ncbi:taxon/001} \arrow[ru, "\texttt{rdfs:subClassOf}" description] &                                                                                                                       &  & \texttt{ncbi:taxon/555}
\end{tikzcd}
